Fairly Allocating Goods in Parallel

We initiate the study of parallel algorithms for fairly allocating indivisible goods among agents with additive preferences. We give fast parallel algorithms for various fundamental problems, such as finding a Pareto Optimal and EF1 allocation under restricted additive valuations, finding an EF1 allocation for up to three agents, and finding an envy-free allocation with subsidies. On the flip side, we show that fast parallel algorithms are unlikely to exist (formally, $CC$-hard) for the problem of computing Round-Robin EF1 allocations.

==> abstract.tex <==
%We consider parallel algorithms for fairly dividing indivisible goods. To this end, we give parallel algorithms that give EF1 and Pareto Optimal (PO) allocations for agents who have restricted additive valuations when there are a bounded number of values. We show that binary valuations are a special case of this and can also be handled by our parallel algorithm. 

%Additionally, we show many related fair division problems also admit efficient parallel solutions. This includes verifying the fairness properties of a given allocation, giving an allocation that is EF-1 and fractionally PO for two additive agents and giving allocations that are EF-1 for up to three additive agents. 

%We show that when we constrain an allocation to respect an ``envy-ordering'' over the agents, parallel algorithms are unlikely to exist. Finally, we show that we can compute fair allocations with envy-eliminating subsidy payments in the style of \cite{HalpernShah2019subsidy} in parallel. Moreover, we can compute \textit{constrained} payment vectors. Constraints can be of the form "Alice should not be paid more than Bob",``Alice should not be paid more than 10 dollars'', etc.


We initiate the study of parallel algorithms for fairly allocating indivisible goods among agents with additive preferences. We give fast parallel algorithms for various fundamental problems, such as finding a Pareto Optimal and EF1 allocation under restricted additive valuations, finding an EF1 allocation for up to three agents, and finding an envy-free allocation with subsidies. On the flip side, we show that fast parallel algorithms are unlikely to exist (formally, \textit{CC}-hard) for the problem of computing Round-Robin EF1 allocations.
